Reasoning for Mobile User Experience with Multimodal LLMs: Task, Benchmark, and Approach

User experience (UX) centered on usability, perceived consistency, and functional clarity is fundamental to real-world user interfaces (UI). The application of multimodal large language models (MLLMs) in the field of user interfaces is evolving rapidly, such as visual element grounding, graphical user interface (GUI) agents, and design-to-code generation. However, research efforts on evaluating UX based on UI screenshots are still immature. To address this, we propose UXBench, a novel multimodal benchmark consisting of 2,000 VQA data samples designed to assess MLLMs' ability to perform UI-based reasoning. UXBench includes 8 tasks based on real-world UI screenshots that require fine-grained diagnosis of UX issues across layout relationships, visual hierarchy, and content consistency. Our extensive evaluation of mainstream MLLMs shows that they remain fundamentally limited in their capacity for UI-based reasoning. The results underscore the need for further advancements in this area. To bridge this gap, we propose UI-UX, an MLLM based on Qwen3-VL-4B-Thinking foundation model and enhanced via reinforcement learning with two key innovations: a reward routing mechanism that dynamically balances perceptual understanding and logical reasoning during inference, and an asymmetric transition reward that suppresses redundant or insufficient reasoning steps. Experiments demonstrate that UI-UX achieves state-of-the-art (SOTA) performance on UXBench, attaining an accuracy of 0.7963 -- surpassing Claude-4.5-Sonnet's 0.6550 -- while exhibiting strong generalization across diverse UI tasks and maintaining low inference latency.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/4_uiux.tex <==
\section{UI-UX}
\label{sec:formatting}

To bridge the significant gap between existing Multimodal Large Language Models (MLLMs) and human experts in user interface (UI) reasoning, we introduce UI-UX, a reinforcement learning-enhanced model specifically optimized for UX diagnostic tasks. Built upon the Qwen-VL-Thinking-4B architecture, UI-UX employs task-aware reinforcement learning (RL) to provide end-to-end guidance for the reasoning generation process, achieving substantial improvements in reasoning efficiency while maintaining diagnostic accuracy.

%-------------------------------------------------------------------------

\subsection{Training Data Composition}

\textbf{Dataset Collection and Annotation.} 
We collect a large-scale dataset of real-world UI screenshots via automated testing scripts executed on eight physical devices spanning Android, HarmonyOS, and iOS. By systematically navigating core user flows in 1,200+ popular applications, we gather 832,432 raw screenshots. To mitigate visual redundancy caused by deterministic execution, we apply perceptual hashing (pHash) and retain only one sample per group of images with Hamming distance $\leq 5$, where the Hamming distance between two pHash ($n$~bit) vectors $\mathbf{h}_i, \mathbf{h}_j \in \{0,1\}^n$ is defined as:

\[
d_H(\mathbf{h}_i, \mathbf{h}_j) = \sum_{k=1}^{n} \mathbb{I}\big[h_i[k] \neq h_j[k]\big],
\]

and $\mathbb{I}[\cdot]$ denotes the indicator function. This yields 68,138 unique UI screenshots.

For scalable, high-fidelity labeling, we propose a two-stage annotation pipeline. First, we leverage multiple MLLMs (GPT5, Gemini2.5-pro, Claude4.5) to predict UX issues across three dimensions (Usability, Efficiency, Content Consistency) and eight sub-tasks, using carefully engineered prompts. Predictions are aggregated via majority voting to generate robust pseudo-labels. Second, all pseudo-labels are manually verified and corrected by five experienced UX researchers, ensuring label accuracy. The resulting dataset, labeled with expert-validated ground truth, enables reliable training and evaluation of UI-aware models for reinforcement learning.

==> uiux/1_intro.tex <==
\section{Introduction}

In modern human-computer interaction systems, the core determinant of success has shifted from functional implementation to the quality of \textbf{User Experience (UX)}\cite{ahmed2025rolelargelanguagemodels}. UI design encompasses the visual and interactive elements of a system, including layout, typography, and screen components, while UX design focuses on the broader user journey, covering the emotional, cognitive, and behavioral responses users experience before, during, and after interacting with the product\cite{bharath2023leader}.The rise of large language models (LLMs) and MLLMs has significantly advanced UX in human-computer interaction. These models enable capabilities such as UI generation~\cite{yang2025uiugunifiedmllmui,lu2023uilayoutgenerationllms,duan2023towards,ran2024guardian}, UI understanding~\cite{you2024ferret,lu2025guiodyssey,lin2025showui}, and user affect recognition~\cite{zhao2025llms,sun2025dialoguemllm,lian2025affectgpt} from raw visual or multimodal inputs, substantially broadening the scope of automated UX analysis. MLLMs facilitate pixel-level interface parsing, intent-driven UI synthesis, and emotion-aware interaction modeling, positioning foundation models as scalable infrastructure for data-driven, user-centric interface systems.

User experience (UX) issues often stem from systematic misalignments between design conventions and user mental models, rather than pixel-level visual anomalies. For instance, a modal dialog occluding navigation bars or inconsistencies between advertised and actual content may appear visually intact, yet cause user frustration, eroded trust, and churn. This paradigm shift, from "perceiving interfaces" to "inferring experiences" poses fundamental challenges for multimodal models in automated UX evaluation.

Despite the growing number of UI-based benchmarks such as Screen2Words \cite{wang2021screen2wordsautomaticmobileui}, Mobile-bench \cite{deng2024mobile}, and VisualWebBench \cite{liu2024visualwebbenchfarmultimodalllms} have been proposed for evaluating UI understanding, they mainly focus on image caption generation, element detection, or layout parsing, essentially visual perception tasks rather than \textbf{UX reasoning}. These benchmarks lack evaluation objectives grounded in behavioral outcomes, cognitive psychology, and trust dynamics. Consequently, they cannot measure models' capability to identify design patterns that may trigger user errors or emotional responses. The absence of user-centric, quantitative, and fine-grained evaluation frameworks fundamentally constrains the applicability of MLLMs to UI design assessment, automated testing, and intelligent design assistance.
\begin{figure*}[t]
\centering
\includegraphics[width=1.02\textwidth, clip, trim=100 545 100 125]{img/yangli.pdf} 
\vspace{-0.3em} 
\label{fig:UXBench samples}
\caption{\textbf{UXBench samples spanning Efficiency, Trustworthiness, and Usability dimensions.} Each case requires visual-semantic reasoning to detect UX defects (e.g., overlapping modals, deceptive content, missing controls). Red bounding boxes indicate ground-truth defect regions for quantitative assessment. Tasks involve inferring experiential consequences beyond pixel-level perception.} 
\vspace{-0.8em} 
\end{figure*}

Some recent studies have attempted to apply MLLMs to UI-related tasks, such as design-to-code generation\cite{yang2025uiugunifiedmllmui}, automated GUI operation (GUI agents), or component recognition. However, these approaches typically rely on manually labeled instruction--action pairs or oversimplify UX issues into binary classification (``good/bad''), overlooking their multi-dimensional, context-dependent, and semantically rich nature. More critically, existing models perform poorly on complex UX defects---e.g., nested pop-ups making operations irreversible, or mismatched service names and page functionalities---often producing vague, erroneous, or contradictory reasoning. This reveals fundamental deficiencies in semantic association, counterfactual reasoning, and intent modeling. Merely aligning vision and text is insufficient for genuine UX understanding; reasoning mechanisms oriented towards human behavior are indispensable.

To address these challenges, we introduce \textbf{UXBench}---the first multimodal benchmark specifically designed to evaluate the UI--UX reasoning capabilities of MLLMs. UXBench contains over 1,900 real UI screenshots and user feedback, systematically decomposing UX issues into three dimensions: usability, efficiency, and trustworthiness, covering 12 fine-grained diagnostic tasks such as insufficient text contrast, pop-up overlapping with capsule area, and badge count inconsistent with message count. Each task is formulated as a two- or three-choice question, requiring models to perform causal reasoning and mapping to design principles rather than keyword matching. Large-scale MLLM-assisted annotation combined with two rounds of expert validation by four senior UX specialists ensures label consistency.


We further propose \textbf{UI-UX}---a reinforcement learning-based MLLM enhancement framework. UI-UX builds upon Qwen3-VL-4B-Thinking\cite{Qwen-VL},\cite{Qwen2-VL},\cite{Qwen2.5-VL} and incorporates a task-adaptive reward routing mechanism: employing answer accuracy as the reward for UX tasks, and ROUGE-L for semantic alignment in general UI understanding tasks. Additionally, we introduce an \textit{overthinking penalty} to dynamically suppress redundant reasoning steps, significantly reducing latency. Without manual preference annotation, our model is optimized end-to-end via the GRPO\cite{shao2024deepseekmathpushinglimitsmathematical} algorithm, achieving 73.8\% accuracy on UXBench and demonstrating strong cross-domain generalization.

\noindent
\textbf{Our contributions are as follows:}
\begin{itemize}
    \item \textbf{First UX reasoning benchmark}: We propose UXBench, defining 11 fine-grained, evaluable, user-centered UI diagnostic tasks, filling a critical gap in the field.
    \item \textbf{Reward routing}: We introduce hard negative sampling and semantic preservation augmentation strategies to address positive sample scarcity and extreme class imbalance in real scenarios.
    \item \textbf{Efficient reasoning}: The proposed UI-UX model combines reward routing and overthinking penalty, achieving MLLM UX reasoning performance surpassing human experts, with low latency and high robustness.
\end{itemize}


==> uiux/3_dataset.tex <==


\section{UXBench}
Existing vision–language benchmarks primarily concentrate on general scene understanding and image generation, they provide insufficient evaluation of models' reasoning and comprehension capabilities in real-world User Interface (UI) contexts. To address this limitation, we present UXBench—the first vision–language benchmark for \textbf{User Experience (UX)} defect diagnosis—designed to systematically assess multimodal large language models (MLLMs) on fine-grained, higher-order reasoning and understanding within realistic UI scenarios.

% \begin{figure}[t]
% \centering
% \includegraphics[width=1.05\columnwidth,trim=50 270 50 250, clip]{img/train_fenbu2.pdf} 
% \caption{fenbu2}
% \label{fig:fenbu2}
% \end{figure}


\subsection{Task Definition}
Traditional UI recognition tasks constitute a form of \textbf{visual perception}, focused on detecting and locating visible interface elements (e.g., buttons, text fields, icons) from screenshots and reconstructing their layout or semantic categories. These approaches rely on explicit visual feature extraction, producing outputs derivable directly from pixel information—following a "recognize objects from images" paradigm—without modeling user behavior or interaction intent. 
In contrast, \textbf{UX diagnosis} tasks require models to not only accurately identify interface components but also evaluate whether their arrangement, interaction logic, and semantic expression pose potential user experience risks. Such issues stem not from isolated element errors but from systematic mismatches between design specifications and human usage conventions. Consequently, UX diagnosis represents a higher-order reasoning task, demanding semantic association and causal inference. For example, determining whether “a popup occludes a button” involves localizing the relevant elements, analyzing spatial relationships and overlap, and inferring if the obstruction impedes intended user actions—ultimately assessing the negative impact on UX. Thus, UX discrimination transcends pixel-level perception, embodying a deeper inference process about interface alignment with human expectations.

For fine-grained evaluation, we decompose UX discrimination into three core dimensions:

\begin{enumerate}
    \item \textbf{Usability}: Measures whether the interface can be correctly understood and effectively operated, focusing on functional discoverability and clarity of interaction feedback.
    \begin{enumerate}[label=(\alph*)]
        \item \textbf{Bubble Occlusion Text (BubbleOcclT)}: Determine whether a must-click-to-close non-modal textual overlay occludes the page’s textual content. Occlusion reduces readability and prevents users from accurately obtaining textual information.
        \item \textbf{Bubble Occlusion Button (BubbleOcclBtn)}: Determine whether a must-click-to-close non-modal textual overlay occludes clickable UI components. Occlusion blocks interactions and prevents users from completing critical actions.
    \end{enumerate}

    \item \textbf{Efficiency}: Evaluates the operational and cognitive cost for users to achieve a goal. Efficient UIs minimize path length and avoid attention interruptions.
    \begin{enumerate}[label=(\alph*)]
        \item \textbf{Popup Without Close Button (PopupNoClose)}: Determine whether a popup provides an explicit close control, restricted to a recognizable “×” icon or a “Close” text button. Without an explicit close control, users struggle to dismiss the popup, causing interruptions and degraded experience.
        \item \textbf{Popup Blocks Native Close Button (PopupBlockClose)}: Identify whether the screenshot is from a mini program and whether an in-page popup affects the clickability of the host interface’s native close button in the top-left/top-right corner. Correct judgment prevents misdiagnosing interaction issues and ensures users can exit via the native close control.
        \item \textbf{Stacked Modal Popups (PopupStack)}: Determine whether two or more modal popups are simultaneously present in the same screen. Stacking popups strongly blocks user operations and increases cognitive load and usage difficulty.
    \end{enumerate}

    \item \textbf{Trustworthiness}: Assesses whether the interface builds and maintains user trust, ensuring information consistency, authoritative communication, and positive emotional tone.
    \begin{enumerate}[label=(\alph*)]
        \item \textbf{Badge-Landing Screen Mismatch (MismatchBadge)}: Judge whether the advertising badge’s copy is consistently baded by the first-screen content of the landing page. Inconsistency causes expectation gaps, user dissatisfaction, and reduced willingness to continue.
        \item \textbf{Service Name-Content Mismatch (MismatchContent)}: Verify that the full service name appears verbatim in the page text and contains no extraneous words absent from the screenshot. Name inconsistency confuses service identity and harms user recognition and trust.
        \item \textbf{Service Description - Functionality Mismatch (MismatchFunc)}: Assess whether the page content matches the core items and details in the service description. Inconsistency misleads user understanding and behavior, damaging trust and overall experience.
    \end{enumerate}
\end{enumerate}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth, clip, trim=80 355 290 325]{img/intro2.pdf}
\caption{intro2}
\vspace{-0.8em} 
\label{fig:pipeline}
\end{figure}


\subsection{Data Pipeline}
UXBench is built through a multi-stage pipeline integrating real user feedback, MLLM-assisted annotation, and human quality control (Fig.~\ref{fig:pipeline}), ensuring authenticity, consistency, and reproducibility.

\textbf{Raw data collection}: Screenshots and textual reports are gathered from in-app feedback of popular mobile apps, covering payment flows, mini-app navigation, subscriptions, etc., naturally reflecting real UX issues.

\textbf{Relevance filtering}: A two-stage classifier filters genuine UX-related cases. Gemini-2.5-Pro labels a subset (relevant/irrelevant), which fine-tunes Qwen3-VL-2B (98\% accuracy). The tuned model processes the corpus at scale, retaining high-confidence positives; negatives are archived.

\textbf{Categorization}: Gemini-2.5-Pro labels positives along three core dimensions—Usability, Efficiency, Trustworthiness—spanning eight subtasks, using few-shot prompting and multi-round voting to resolve ambiguities.

\textbf{Human verification}: Four senior UX researchers conduct two-stage manual checks: (1) verify dimension labels for all positives; (2) cross-check a random 20\% subset for reliability.

\textbf{Final dataset}: Balanced sampling yields 100 samples per option for each subtask from positives, plus balanced negatives. Final set: 1,900 high-quality image–question pairs covering both defects and normal cases.

\subsection{Data Distribution}
UXBench ensures balanced, diverse task distribution, option design, and platforms.

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth, trim=350 200 350 230, clip]{img/fenbu.pdf} 
\caption{Data distribution by subtask.}
\vspace{-0.8em} 
\label{fig:fenbu}
\end{figure}

\textbf{Task distribution}: 1,900 tasks across three dimensions (500/600/800 samples), with 2, 3, 3 subtasks respectively (Fig.~\ref{fig:fenbu}). Each subtask has 200–300 balanced positive/negative samples.

\textbf{Option count}: Multiple-choice format—2 options: 42\% (800), 3 options: 58\% (1,100).

\textbf{Platform coverage}: Includes iOS/Android, light/dark themes, portrait/landscape orientations for better real-world generalization.


==> uiux/7_acknowledgments.tex <==
\section*{Acknowledgments}

This work was supported by Ant Group.
We thank the anonymous reviewers for their thoughtful feedback
which greatly improved this work.
